Electric routing and concurrent flow cutting

We investigate an oblivious routing scheme, amenable to distributed computation and resilient to graph changes, based on electrical flow. Our main technical contribution is a new rounding method which we use to obtain a bound on the L1->L1 operator norm of the inverse graph Laplacian. We show how this norm reflects both latency and congestion of electric routing.

==> latency.tex <==

\subsection{Latency}

The expected number of edges traversed between $s$ and $t$
reflects the routing latency.
Using the machinery we've developed so far, it is quite easy to establish
(Proven in Appendix~\ref{sec:latency-proof}):
%
\begin{theorem}\label{theo:stretch}
The latency of every electric walk on an undirected 
graph of bounded degree $d_{\max}$ 
and vertex expansion $\alpha$
is at most $O(\min\{n^{1/2},d_{\max}\alpha^{-2}\ln n \})$.
\end{theorem}
%
For expanders, this theorem is not trivial. In fact, there exist
path realizations of the electric walk which can traverse up to $O(n)$ edges.
Theorem~\ref{theo:stretch} asserts that this happens with small probability. On
the other hand, in a bounded-degree expander, even if $s$ and $t$ are adjacent
the walk will still take a $O(\log n)$-length path with constant probability.
%

